A High-Order Shifted Interface Method for Lagrangian Shock Hydrodynamics

We present a new method for two-material Lagrangian hydrodynamics, which combines the Shifted Interface Method (SIM) with a high-order Finite Element Method. Our approach relies on an exact (or sharp) material interface representation, that is, it uses the precise location of the material interface. The interface is represented by the zero level-set of a continuous high-order finite element function that moves with the material velocity. This strategy allows to evolve curved material interfaces inside curved elements. By reformulating the original interface problem over a surrogate (approximate) interface, located in proximity of the true interface, the SIM avoids cut cells and the associated problematic issues regarding implementation, numerical stability, and matrix conditioning. Accuracy is maintained by modifying the original interface conditions using Taylor expansions. We demonstrate the performance of the proposed algorithms on established numerical benchmarks in one, two and three dimensions.

==> SBM.tex <==
%--------------
%\subsection{Weak discrete formulation}
%
%Let us consider~\eqref{mom}--\eqref{ene} and test them agains some arbitrary test functions $\phi$ and $\bs{\psi}$. Namely
%
%In deriving the shifted DG formulation, we will follow the typical steps of the local discontinuous Galerkin (LDG) formulation (see, e.g.,~\cite{arnold2002unified}, for more details). Multiplying the strong form of the equations~\eqref{mom}--\eqref{ene}
%by the test function pair $[\phi \, , \, \bs{\psi}]$ and integrating over the generic element $T$ of the finite element mesh yield
%%
%\begin{subequations}
%	\begin{align}
%	(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{T}
%	+ 	(\bs{\psi} \, , \, \nabla p )_{T}
%	=
%	(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{T}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{T}
%	&
%	+  \langle p\, , \, \bs{\psi}\cdot \bs{n}  \rangle _{\partial T}
%	= 0
%	\, , \\
%	(\phi \, , \, \rho \dot{e} )_{T}
%	+
%	(\phi \, , \, p \, \nabla \cdot  \bs{v} )_{T}
%	& =
%	(\phi \, , \, \rho \dot{e} )_{T}
%	- ( \nabla (\phi \, p) \, , \,   \bs{v} )_{T}
%	+\langle\bs{v}\cdot\bs{n} \, , \, \phi \, p \rangle_{\partial T}
%	= \;
%	0
%	\,.
%	\end{align}
%\end{subequations}
%%
%Replacing the boundary traces by suitable \textit{numerical fluxes}, $\hat{p}$ and $\hat{\bs{v}}$, yields
%%
%\begin{subequations}
%	\begin{align}
%	(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{T}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{T}
%	+  \langle \hat{p}\, , \, \bs{\psi}\cdot\bs{n}  \rangle_{\partial T}
%	& = \;
%	0
%	\, , \\
%	(\phi \, , \, \rho \dot{e} )_{T}
%	- ( \nabla (\phi \, p) \, , \,   \bs{v} )_{T}
%	+\langle \hat{\bs{v}}\cdot\bs{n} \, , \, \phi \, p \rangle_{\partial T}
%	& = \;
%	0\,.
%	\end{align}
%\end{subequations}
%%
%The numerical fluxes $\hat{p}$ and $\hat{\bs{v}}$ accomplish the linking of the numerical solution between neighboring elements, and will be defined momentarily. Summing over all the elements and integrating back by parts the second equation we have
%%
%\begin{subequations}
%	\label{eq:baseDGO1}
%	\begin{align}
%	(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\sum_{T \in \ti{\mathcal{T}}^h} \langle \hat{p}\, , \, \bs{\psi}\cdot\bs{n}  \rangle _{\partial T}
%	& = \;
%	0
%	\, , \\
%	(\phi \, , \, \rho \dot{e} )_{\Om}
%	+ ( \nabla \cdot \bs{v} \, , \,   \phi \, p )_{\Om}
%	+\sum_{T \in \ti{\mathcal{T}}^h} \langle \hat{\bs{v}} \cdot \bs{n} \, , \, \phi \, p  \rangle _{\partial T}
%	- \sum_{T \in \ti{\mathcal{T}}^h} \langle \bs{v} \cdot \bs{n} \, , \, \phi \, p  \rangle _{\partial T}
%	& = \;
%	0\,.
%	\end{align}
%\end{subequations}
%%
%%
%%
%%
%Next, we introduce the average operator $\avgb{ \cdot}_\gamma $ and the jump operator $\jump{\cdot}$
%for discontinuous scalars, vector and tensor fields across element boundaries:
%\begin{subequations}
%	\label{eq:jump_avgO1}
%	\begin{align}
%	\avgb{ p}_{\gamma}
%	&=\;
%	\gamma \, p^{+}+(1-\gamma ) \, p^{-}
%	\, , \, &
%	\avgb{ \bs{v}}_{\gamma}
%	&=\;
%	\gamma \,\bs{v}^{+}+(1-\gamma ) \,\bs{v}^{-}
%	\, ,  \, &
%	\avgb{ \bs{M}}_{\gamma}
%	&=\;
%	\gamma \,\bs{M}^{+}+(1-\gamma ) \,\bs{M}^{-}
%\, , \quad  \forall \gamma \in [0,1]
%	\, , \\
%	\jump{p}
%	&=
%	p^{+}\bs{n}^{+}+p^{-}\bs{n}^{-}
%	\, , \, &
%	\jump{\bs{v}}
%	&=\; \bs{v}^{+}\cdot\bs{n}^{+}+\bs{v}^{-}\cdot\bs{n}^{-}
%	\, , \, &
%	\jump{\bs{M}}
%	&=\; \bs{M}^{+}\bs{n}^{+}+\bs{M}^{-}\bs{n}^{-}
%	\end{align}
%\end{subequations}
%%
%where $\bs{n}^{+}$ and $\bs{n}^{-}$  indicate opposite normals to a face.
%A reordering argument yields
%%
%\begin{equation}
%\sum_{T \in \ti{\mathcal{T}}^h} \avg{w\, , \, \bs{v}\cdot\bs{n} } _{\partial T}
%=
%\avg{ \avgb{ w }_{\gamma} \, , \, \jump{\bs{v}} }_{\tGI}
%+
%\avg{ \jump{ w } \, , \, \avgb{ \bs{v}}_{1-\gamma} }_{\tGI }
%+
%\avg{ w \, \bs{n} \, , \, \bs{v} } _{\G}
%\, ,
%\label{eq: identity propertyO1}
%\end{equation}
%%
%Using the definitions~\eqref{eq:jump_avgO1} of jump and average operators and inserting identity~\eqref{eq: identity propertyO1} into~\eqref{eq:baseDGO1}, we obtain
%%
%\begin{subequations}
%	\label{eq:dg_bf_intermediateO1}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_1O1}
%	&(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\avg{ \avgb{ \hat{p}}_{\gamma} \, , \, \jump {\bs{\psi}} }_{\tGI}
%	+\avg{ \jump{ \hat{p}} \, , \, \avgb{ \bs{\psi}}_{1-\gamma} } _{\tGI}
%	+\avg{ \hat{p}\, , \, \bs{\psi} \cdot \bs{n} }_{\G}
%	= \;
%	0
%	\,,\\
%	\label{eq:dg_bf_intermediate_2O1}
%	&(\phi \, , \, \rho \dot{e} )_{\Om}
%	+ ( \nabla \cdot \bs{v} \, , \,   \phi \, p )_{\Om}
%	+\avg{ \jump {\hat{\bs{v}} } \, , \,  \avgb{ \phi \, p }_{\gamma} }_{\tGI }
%	+\avg{  \avgb{\hat{\bs{v}}}_{1-\gamma}\, , \, \jump{ \phi \, p } }_{\tGI }
%	\nonumber \\
%	& \phantom{=}
%	-\avg{ \jump {\bs{v} } \, , \,  \avgb{ \phi \,p }_{\gamma} }_{\tGI }
%	-\avg{  \avgb{\bs{v}}_{1-\gamma}\, , \, \jump{ \phi \, p } }_{\tGI }
%	+\avg{  (\hat{\bs{v}} - \bs{v})  \cdot \bs{n} \, , \,  \phi \, p }_{\G}
%	= \;
%	0
%	\, .
%	\end{align}
%\end{subequations}
%%
%%
%The sum of these equations will constitute the basis of the variational formulation.
%%
%
%%-------
%
%\paragraph{Enforcing interface conditions}
%Note that the surrogate normal $\bs{\tilde{n}}$ can be written as
%\begin{equation}
%\bs{\tilde{n}} = \left( \bs{\tilde{n}} \cdot \bs{n} \right) \bs{n} +
%                 \left( \bs{\tilde{n}} \cdot \bs{\tau_i} \right) \bs{\tau_i},
%\end{equation}
%thus, for the surrogate velocity $\bs{v}$, we can write
%\begin{equation}
%\bs{v} \cdot \bs{\tilde{n}} =
%  \bs{v} \cdot \bs{n} \left( \bs{\tilde{n}} \cdot \bs{n} \right) +
%  \bs{v} \cdot \bs{\tau_i} \left( \bs{\tilde{n}} \cdot \bs{\tau_i} \right),
%\quad
%\jump{\bs{v}} =
%  \jump{ (\bs{v} \cdot \bs{n}) \bs{n} +
%         (\bs{v} \cdot \bs{\tau_i}) \bs{\tau_i} }.
%\end{equation}
%Next, recall that the interface condition at the true interface
%(using a Taylor expansion) is
%\[
%(\bs{v}^+ + \nabla \bs{v}^+ \bs{d} ) \cdot \bs{n} =
%(\bs{v}^- + \nabla \bs{v}^- \bs{d} ) \cdot \bs{n}.
%\]
%Then we can replace the use of $(\bs{v} \cdot \bs{n})$ in the following way:
%\[
%\jump{ (\bs{v} \cdot \bs{n}) \bs{n} } =
%\bs{v}^+ \cdot \bs{n} - \bs{v}^- \cdot \bs{n} =
%(\nabla \bs{v}^- \bs{d}) \cdot \bs{n} - (\nabla \bs{v}^+ \bs{d}) \cdot \bs{n} =
%- \jump{((\nabla \bs{v} \bs{d}) \cdot \bs{n}) \bs{n}}
%\]
%With these, the interface conditions for $p$ and $\bs{v}$ can be reflected through
%\begin{equation}
%\begin{aligned}
%\jump{\hat{p}} &= - \jump{\nabla p \cdot \bs{d}} \\
%\jump{\hat{\bs{v}}} &= - \jump{ ((\nabla \bs{v} \bs{d}) \cdot \bs{n}) \bs{n} -
%                                (\bs{v} \cdot \bs{\tau_i}) \bs{\tau_i} } \\
% \avgb{\hat{p}}_{\gamma} &= \avgb{p}_{\gamma} \\
%  \avgb{\hat{\bs{v}}}_{1-\gamma} &=   \avgb{\bs{v}}_{1-\gamma}
%\end{aligned}
%\end{equation}
%%
%%
%\begin{comment}
%Applying the LDG-type flux definitions~\cite{arnold2002unified} as a reference,
%we define the following {\it shifted} numerical fluxes on $\tGI$,
%%
%
%\begin{equation}
%\begin{aligned}
%\hat{p}^{+}
%&=
%\avgb{ p}_{\gamma}
%- (1-\gamma) \, \left( \jump{ \nabla p\cdot \bs{d} } \cdot \ti{\bs{n}}^{+} \right)
%\; ,   \\
%\hat{p}^{-}
%&=
%\hat{p}^{+}
%+  \jump{ \nabla p \cdot \bs{d} } \cdot \ti{\bs{n}}^{+}
%\; ,   \\
%\hat{\bs{v}}^{+}
%&=
%\avgb{ \bs{v}}_{1-\gamma}
%- \gamma \jump{\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n} -  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i}  } \ti{\bs{n}}^{+}
%\; , \\
%\hat{\bs{v}}^{-}
%&=
%\hat{\bs{v}}^{+}
%+ \jump{\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n}
%	-  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i}  } \ti{\bs{n}}^{+}
%\, .
%%\end{array}
%\end{aligned}
%\end{equation}
%where $\bs{\tau}_i$ as a unit vector tangent to the true boundary surface (and we imply repeated index notation). In addition, we define $\hat{p}  = p$ and $\hat{\bs{v}} = t_{I} \,\bs{n}$ on $\G$.
%\end{comment}
%
%%-------
%
%\paragraph{Shifted discrete variational form}
%
%Once the above substitutions are made, the {\it discrete} variational form reads
%\begin{subequations}
%	\label{eq:dg_bf_intermediate_3O1}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_4O1}
%	&(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\avg{ \avgb{ p}_{\gamma} \, , \, \jump {\bs{\psi}} }_{\tGI}
%	-\avg{ \jump{ \nabla p \cdot \bs{d} }  \, , \, \avgb{ \bs{\psi}}_{1-\gamma} } _{\tGI}
%	+\avg{ p\, , \, \bs{\psi} \cdot \bs{n} }_{\G}
%	= \;
%	0
%	\,,\\
%	\label{eq:dg_bf_intermediate_5O1}
%	&(\phi \, , \, \rho \dot{e} )_{\Om}
%	+ ( \nabla \cdot \bs{v} \, , \,   \phi \, p )_{\Om}
%	-\avg{ \jump {\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n}
%			-  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i} } \, , \,  \avgb{ \phi \, p }_{\gamma} }_{\tGI }
%	-\avg{ \jump {\bs{v} } \, , \,  \avgb{ \phi \,p }_{\gamma} }_{\tGI }
%	-\avg{  \bs{v} \cdot \bs{n} \, , \,  \phi \, p }_{\G}
%	= \;
%	0
%	\, ,
%	\end{align}
%\end{subequations}
%%and the discrete trial and test spaces~\eqref{eq:finite_dimensional_function_spaces_Darcy} are introduced,
%which can be rewritten as,
%\begin{subequations}
%	\label{eq:dg_bf_intermediate_6O1}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_7O1}
%	&(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\avg{ \avgb{ p}_{\gamma} \, , \, \jump {\bs{\psi}} }_{\tGI}
%	-\avg{ \jump{ \nabla p \cdot \bs{d} } \, , \, \avgb{ \bs{\psi}}_{1-\gamma} } _{\tGI}
%	+\avg{ p\, , \, \bs{\psi} \cdot \bs{n} }_{\G}
%	= \;
%	0
%	\,,\\
%	\label{eq:dg_bf_intermediate_8O1}
%	&(\phi \, , \, \rho \dot{e} )_{\Om}
%	+ ( \nabla \cdot \bs{v} \, , \,   \phi \, p )_{\Om}
%	-\avg{ \jump {\bs{n} \otimes \bs{n} \,\, \bs{S}^{h} \bs{v}} \, , \,   \avgb{\phi \, p }_{\gamma}  }_{\tGI }
%		-\avg{  \bs{v} \cdot \bs{n} \, , \,  \phi \, p }_{\G}
%	= \;
%	0
%	\, .
%	\end{align}
%\end{subequations}
%{\color{red}To ensure full continuity of the velocity we can also add a penalty term on the tangential component given as: $ \avg{ \alpha \, \tau  \, \jump{ ( \mathbb{I} - \bs{n} \otimes \bs{n} )  \, (\bs{S}^{h} \bs{v} \otimes \ti{\bs{n}}^{+})}  \, , \, \jump{ ( \mathbb{I} - \bs{n} \otimes \bs{n} )  \, (\bs{S}^{h} \bs{\psi} \otimes \ti{\bs{n}}^{+}) } }_{\tGI}$
%where $\alpha = \beta \, (( \mathbb{I} - \bs{n}^{+} \otimes \bs{n}^{+} ):( \mathbb{I} - \ti{\bs{n}}^{+} \otimes \ti{\bs{n}}^{+} ))^{2} $, $\beta$ is a positive constant independent of the mesh, $\tau =  \frac{2 \, (\rho \, c_{s})^{+}(\rho \, c_{s})^{-}}{ (\rho \, c_{s})^{+}+(\rho \, c_{s})^{-}}$ with $c_{s}^{\pm}$ being the speed of sound on either side of an interior interface edge. }
%
%{\gs
%
%\subsubsection{Multiple interfaces}
%If multiple materials are present and multiple interfaces need to be characterized, the previous formulation can be extended as follows
%\begin{subequations}
%	\label{eq:dg_bf_intermediate_6O1_multiple}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_7O1_multiple}
%	&\sum_{j=1}^{N_{\Om}}  (\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\ti{\Om}_j}
%	- \sum_{j=1}^{N_{\Om}}  (\nabla \cdot \bs{\psi} \, , \,  p )_{\ti{\Om}_j}
%	+\sum_{k=1}^{N_I} \avg{ \avgb{ p}_{\gamma} \, , \, \jump {\bs{\psi}} }_{\tGIk}
%	-\sum_{k=1}^{N_I} \avg{ \jump{ \nabla p \cdot \bs{d} } \, , \, \avgb{ \bs{\psi}}_{1-\gamma} } _{\tGIk}
%	+\avg{ p\, , \, \bs{\psi} \cdot \bs{n} }_{\G}
%	= \;
%	0
%	\,,\\
%	\label{eq:dg_bf_intermediate_8O1_multiple}
%	& \sum_{j=1}^{N_{\Om}} (\phi \, , \, \rho \dot{e} )_{\ti{\Om}_j}
%	+ \sum_{j=1}^{N_{\Om}} ( \nabla \cdot \bs{v} \, , \,   \phi \, p )_{\ti{\Om}_j}
%	-\sum_{k=1}^{N_I} \avg{ \jump {\bs{n} \otimes \bs{n} \,\, \bs{S}^{h} \bs{v}} \, , \,   \avgb{\phi \, p }_{\gamma}  }_{\tGIk}
%	-\avg{  \bs{v} \cdot \bs{n} \, , \,  \phi \, p }_{\G}
%	= \;
%	0
%	\, ,
%	\end{align}
%\end{subequations}
%where $N_{\Om}$ is the number of separate material domains and $N_I$ is the number of material interfaces.
%
%
%
%
%\subsubsection{Formulation for a strongly continuous velocity}
%In the case a continuous space is chosen for the velocity, the previous formulation further simplifies. Assuming that normal velocity boundary conditions are applied strongly on $\G$, we have:
%\begin{subequations}
%	\label{eq:dg_bf_intermediate_6O1_multiple_strong}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_7O1_multiple}
%	&\sum_{j=1}^{N_{\Om}}  (\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\ti{\Om}_j}
%	- \sum_{j=1}^{N_{\Om}}  (\nabla \cdot \bs{\psi} \, , \,  p )_{\ti{\Om}_j}
%	-\sum_{k=1}^{N_I} \avg{ \jump{ \nabla p \cdot \bs{d} } \, , \, \bs{\psi} } _{\tGIk}
%	= \;
%	0
%	\,,\\
%	\label{eq:dg_bf_intermediate_8O1_multiple_strong}
%	& \sum_{j=1}^{N_{\Om}} (\phi \, , \, \rho \dot{e} )_{\ti{\Om}_j}
%	+ \sum_{j=1}^{N_{\Om}} ( \nabla \cdot \bs{v} \, , \,   \phi \, p )_{\ti{\Om}_j}
%	-\sum_{k=1}^{N_I} \avg{ \jump {\bs{n} \otimes \bs{n} \,\, \bs{S}^{h} \bs{v}} \, , \,   \avgb{\phi \, p }_{\gamma}  }_{\tGIk}
%	= \;
%	0
%	\, ,
%	\end{align}
%\end{subequations}
%
%
%
%
%}
%
%\subsubsection{Conservation properties}
%
%It is important at this point in the discussion to analyze conservation statements for the Shifted Interface Method.
%
%To start the discussion, let us consider a body-fitted variational formulation that corresponds to the limit case of the Shifted Interface Method when $\bs{d} \rightarrow \bs{0}$, so that $\tGI \rightarrow \G_I$, $\ti{\bs{n}} \rightarrow \bs{n}$, $\ti{\bs{n}} \cdot \bs{n} = 1$ and $\ti{\bs{n}} \cdot \bs{\tau}_i = 0$.
%In this limit, \eqref{eq:dg_bf_intermediate_6O1} reduce to:
%%
%\begin{subequations}
%	\label{eq:SH_Cons1}
%	\begin{align}
%	(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	-
%	(\nabla \cdot \bs{\psi} \, , \, p )_{\Om}
%	+\avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{\psi} }  }_{\G_I}
%	&=\;
%	0 \; ,
%	\\
%	(\phi \, , \, \rho \dot{e} )_{\Om}
%	+( \phi \, , \,  p \, \nabla \cdot \bs{v} )_{\Om}
%	- \avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{\bs{v} } }_{\G_I}
%	&=\;
%	0 \; .
%	\end{align}
%\end{subequations}
%%
%Setting $\phi=0$, $\bs{\psi}=\bs{e}_i$ (where $\bs{e}_i$ is the unit vector along the $i$th coordinate axis) and applying~\eqref{mass} twice yields the conservation of momentum statement:
%%
%\begin{subequations}
%	\label{eq:SH_Cons2_gen}
%	\begin{align}
%	\label{eq:SH_Cons2}
%	(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	=
%	\partial_t (1 \, , \, \rho \bs{v} \cdot \bs{e}_i)_{\Om}
%	&=\;
%	0 \; , \qquad i=1, \ldots , d
%	\end{align}
%	which states that global integral of the momentum is conserved over time for the semi-discrete system of equations.
%	The global statement of conservation of total energy is obtained setting $\phi=1$ in the energy equation, $\bs{\psi}=\bs{v}$ in the momentum equation (to obtain a kinetic energy balance), and summing the results:
%	%
%	\begin{align}
%	\label{eq:SH_Cons3a}
%	\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%	&=\;
%	(\nabla \cdot \bs{v} \, , \, p )_{\Om}
%	-\avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{v} }  }_{\G_I}
%	-( 1 \, , \,  p \, \nabla \cdot \bs{v} )_{\Om}
%	+ \avg{ \avgb{ p }_\lambda \, , \,    \jump{\bs{v} } }_{\G_I},
%	\end{align}
%	which can be recast as
%	\begin{align}
%		\label{eq:SH_Cons3}
%	\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%	+ (1 \, , \, \nabla \cdot( \bs{v} \, p) )_{\Om}
%	&= \;
%	\avg{ \jump{ p }  \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\G_I}
%	+ \avg{ \jump{ \bs{v} }  \, , \, \avgb{ p }_\lambda  }_{\G_I}
%	= 0
%	\end{align}
%\end{subequations}
%%
%
%The case of the Shifted Interface Method is different, and in general it will not be possible to observe cancellation of fluxes over $\tGI$similar to the ones over $\G_I$ in~\eqref{eq:SH_Cons2}--\eqref{eq:SH_Cons3}.
%This is because the SIM attempts to find approximations to the interface conditions on the true interface $\G_I$ using Taylor expansions of the field centered at points on $\tGI$. Analogously, setting $\phi=1$ in the energy equation and $\bs{\psi}=\bs{v}$ in the momentum equation, we obtain
%\begin{subequations}
%	%
%	\begin{align}
%	\label{eq:SH_Cons4b}
%	\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%	&=\;
%	\avg{ \jump{(\nabla p ) \bs{d}}   \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%	%
%	+ \avg{ \avgb{ p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, ( (\nabla \bs{v}) \bs{d}) - (\bs{\tau}_i \otimes \bs{\tau}_i) \, \bs{v}} }_{\tGI}
%	\; ,
%	\nonumber \\
%	& = \;
%	\avg{ \jump{p + (\nabla p ) \bs{d}}   \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%	%
%	+\avg{ \avgb{  p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, (\bs{v} + (\nabla \bs{v}) \bs{d}) } }_{\tGI}
%	\nonumber \\
%	& \phantom{=} \;
%	- \avg{ \jump{ p } \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%	- \avg{ \avgb{ p }_\lambda \, , \,    \jump{ \bs{v} } }_{\tGI}
%	\end{align}
%	%
%	which can be recast as
%	%
%	\begin{align}
%	\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%	+ (1 \, , \, \nabla \cdot( \bs{v} \, p) )_{\Om}
%	& = \;
%	\avg{ \jump{p + (\nabla p ) \bs{d}}  \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%	%\nonumber \\
%	%& \phantom{=} \;
%	+\avg{ \avgb{ p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, (\bs{v} + (\nabla \bs{v}) \bs{d}) }  }_{\tGI}
%	\nonumber \\
%	& = \;
%	O(h^2)
%	\end{align}
%\end{subequations}
%which indicates that a small, order $O(h^2)$, perturbation to the energy balance needs to be imposed to enforce the matching conditions~\eqref{eq:SBM_SH_IP}--\eqref{eq:SBM_SH_IN}.
%This is of course expected, since the Taylor expansion is truncated to respect second-order accuracy.
%
%
%%--------------
%
%%--------------
%
%%\subsection{Shifted variational formulation}
%%
%%Let us consider~\eqref{mom}--\eqref{ene} and test them agains some arbitrary test functions $\phi$ and $\bs{\psi}$. Namely
%%\begin{subequations}
%%\label{eq:SH_Weak2}
%%\begin{align}
%%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%%+
%%(\bs{\psi} \, , \, \nabla p )_{\Om}
%%&=\;
%%0 \; ,
%%\\
%%(\phi \, , \, \rho \dot{e} )_{\Om}
%%+
%%(\phi \, , \, p \, \nabla \cdot  \bs{v} )_{\Om}
%%&=\;
%%0 \; .
%%\end{align}
%%\end{subequations}
%%%
%%Integrating by parts, and omitting the terms on the outer boundary $\G$, we obtain
%%%
%%\begin{subequations}
%%\label{eq:SH_Weak3}
%%\begin{align}
%%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%%-
%%(\nabla \cdot \bs{\psi} \, , \, p )_{\Om}
%%+\avg{ 1 , \jump{\bs{\psi} \, p} }_{\tGI}
%%&=\;
%%0 \; ,
%%\\
%%(\phi \, , \, \rho \dot{e} )_{\Om}
%%-(\nabla ( \phi \, p) \, , \, \bs{v} )_{\Om}
%%+\avg{ 1 , \jump{ \phi \, p \, \bs{v} } }_{\tGI}
%%&=\;
%%0 \; .
%%\end{align}
%%\end{subequations}
%%%
%%We now define the $\lambda$-weighted average $\avgb{w}_\lambda = \lambda w^+ + (1-\lambda) w^-$ of a quantity $w$ for any $\lambda \in[0, 1]$ and note the identity $ \ljump{ \phi \, \bs{\psi} } =  \avgb{ \phi }_\lambda \ljump{ \bs{\psi} } + \ljump{ \phi } \cdot  \avgb{ \bs{\psi} }_{1-\lambda} $, so that~\eqref{eq:SH_Weak3} yields
%%%
%%\begin{subequations}
%%\label{eq:SH_Weak4}
%%\begin{align}
%%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%%-
%%(\nabla \cdot \bs{\psi} \, , \, p )_{\Om}
%%+\avg{ 1 ,  \avgb{ p }_\lambda \ljump{ \bs{\psi} } + \ljump{ p } \cdot  \avgb{ \bs{\psi} }_{1-\lambda}  }_{\tGI}
%%&=\;
%%0 \; ,
%%\\
%%(\phi \, , \, \rho \dot{e} )_{\Om}
%%-(\nabla ( \phi \, p) \, , \, \bs{v} )_{\Om}
%%+\avg{ 1 ,  \avgb{ \phi \, p }_\lambda \ljump{ \bs{v} } + \ljump{ \phi \, p } \cdot  \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%%&=\;
%%0 \; .
%%\end{align}
%%\end{subequations}
%%%
%%Note now that condition~\eqref{eq:SBM_SH_IP} can be rewritten as $\jump{p} = - \jump{(\nabla p ) \bs{d}} $ on $\tGI$.
%%Hence:
%%%
%%\begin{subequations}
%%\label{eq:SH_Weak5}
%%\begin{align}
%%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%%-
%%(\nabla \cdot \bs{\psi} \, , \, p )_{\Om}
%%+\avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{\psi} }  }_{\tGI}
%%- \avg{ \jump{(\nabla p ) \bs{d}} \, , \,   \avgb{ \bs{\psi} }_{1-\lambda}  }_{\tGI}
%%&=\;
%%0 \; ,
%%\\
%%\label{eq:SH_Weak5b}
%%(\phi \, , \, \rho \dot{e} )_{\Om}
%%-(\nabla ( \phi \, p) \, , \, \bs{v} )_{\Om}
%%+\avg{ \avgb{ \phi \, p }_\lambda \, , \,    \ljump{ \bs{v} } }_{\tGI}
%%+\avg{ \ljump{ \phi \, p } \, , \,  \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%%&=\;
%%0 \; .
%%\end{align}
%%\end{subequations}
%%%
%%Observe now the decomposition of the identity tensor $\bs{I} = \bs{n} \otimes \bs{n} + \bs{\tau}_i \otimes \bs{\tau}_i$ where Einstein repeated index notation is applied to the sum of dyadic products $\bs{\tau}_i \otimes \bs{\tau}_i$.
%%Now, \eqref{eq:SBM_SH_IN} can be rewritten as $\jump{ (\bs{n} \otimes \bs{n}) \, \bs{v} } = - \jump{ ( \bs{n} \otimes \bs{n} )  \, (\nabla \bs{v}) \bs{d} }$, and
%%%
%%\begin{subequations}
%%\label{eq:SH_Weak6}
%%\begin{align}
%%\avg{ \avgb{ \phi \, p }_\lambda \, , \,    \ljump{ \bs{v} } }_{\tGI}
%%=
%%- \avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, (\nabla \bs{v}) \bs{d} } }_{\tGI}
%%+\avg{ \avgb{ \phi \, p }_\lambda \, , \,   \jump{ (\bs{\tau}_i \otimes \bs{\tau}_i) \, \bs{v} }  }_{\tGI}
%%\; .
%%\end{align}
%%\end{subequations}
%%%
%%Integrating back by parts~\eqref{eq:SH_Weak5b}, we obtain the final variational form
%%%
%%\begin{subequations}
%%\label{eq:SH_Weak7}
%%\begin{align}
%%\label{eq:SH_Weak7a}
%%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%%-(\nabla \cdot \bs{\psi} \, , \, p )_{\Om}
%%+\avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{\psi} }  }_{\tGI}
%%- \avg{ \jump{(\nabla p ) \bs{d}} \, , \,   \avgb{ \bs{\psi} }_{1-\lambda}  }_{\tGI}
%%&=\;
%%0 \; ,
%%\\
%%\label{eq:SH_Weak7b}
%%(\phi \, , \, \rho \dot{e} )_{\Om}
%%+( \phi \, , \,  p \, \nabla \cdot \bs{v} )_{\Om}
%%- \avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, (\bs{v} + (\nabla \bs{v}) \bs{d}) } }_{\tGI}
%%%{\color{cyan}
%%%+ \avg{ \jump{p+(\nabla p ) \bs{d}} \, , \,   \avgb{ \phi \, \bs{v} }_{1-\lambda}  }_{\tGI}
%%%}
%%&=\;
%%0 \; .
%%\end{align}
%%\end{subequations}
%%%
%%\begin{remark}
%%The set of equations~\eqref{eq:SH_Weak7} is written in the current configuration of the domain, involving $\Om$ and $\G_I$, that is need to be integrated on a moving grid.
%%In order to compute $\bs{d}$, one needs in principle to update in time $\G_I$, which may be seen as an unwanted complication.
%%Alternatively, the distance vector can be updated as $\bs{d} = \mathbf{Cof}[\bs{F}] \, \bs{D}$, in which $\bs{D}=\bs{d}(\bs{x},t=0)$ is the distance vector computed at the initial configuration of the material body.
%%The idea is to evaluate $\bs{D}$ at the beginning of the computation, and then use the formula $\bs{d} = \mathbf{Cof}[\bs{F}] \, \bs{D}$ on the surrogate interface, at every time and location when $\bs{d}$ needs to be evaluated.
%%A third option is to pull back the system of equations~\eqref{eq:SH_Weak7} to the reference (original) configuration, involving $\Om_0$, $\G_{I;0}$, etc., and to implement the shifted boundary/interface approach in this setting, in which the geometry does not change.
%%Note that the last two approaches described are effectively equivalent, and the specific choice of one versus the other is typically incidental.
%%\end{remark}
%%
%%%-------
%%
%%\subsection{Conservation properties}
%%
%%It is important at this point in the discussion to analyze conservation statements for the Shifted Interface Method.
%%
%%To start the discussion, let us consider a body-fitted variational formulation that corresponds to the limit case of the Shifted Interface Method when $\bs{d} \rightarrow \bs{0}$, so that $\tGI \rightarrow \G_I$, $\ti{\bs{n}} \rightarrow \bs{n}$, $\ti{\bs{n}} \cdot \bs{n} = 1$ and $\ti{\bs{n}} \cdot \bs{\tau}_i = 0$.
%%In this limit, \eqref{eq:SH_Weak7} reduce to:
%%%
%%\begin{subequations}
%%\label{eq:SH_Cons1}
%%\begin{align}
%%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%%-
%%(\nabla \cdot \bs{\psi} \, , \, p )_{\Om}
%%+\avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{\psi} }  }_{\G_I}
%%&=\;
%%0 \; ,
%%\\
%%(\phi \, , \, \rho \dot{e} )_{\Om}
%%+( \phi \, , \,  p \, \nabla \cdot \bs{v} )_{\Om}
%%- \avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{\bs{v} } }_{\G_I}
%%&=\;
%%0 \; .
%%\end{align}
%%\end{subequations}
%%%
%%Setting $\phi=0$, $\bs{\psi}=\bs{e}_i$ (where $\bs{e}_i$ is the unit vector along the $i$th coordinate axis) and applying~\eqref{mass} twice yields the conservation of momentum statement:
%%%
%%\begin{subequations}
%%\label{eq:SH_Cons2_gen}
%%\begin{align}
%%\label{eq:SH_Cons2}
%%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%%=
%%\partial_t (1 \, , \, \rho \bs{v} \cdot \bs{e}_i)_{\Om}
%%&=\;
%%0 \; , \qquad i=1, \ldots , d
%%\end{align}
%%which states that global integral of the momentum is conserved over time for the semi-discrete system of equations.
%%The global statement of conservation of total energy is obtained setting $\phi=1$ in the energy equation, $\bs{\psi}=\bs{v}$ in the momentum equation (to obtain a kinetic energy balance), and summing the results:
%%%
%%\begin{align}
%%\label{eq:SH_Cons3a}
%%\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%%&=\;
%%(\nabla \cdot \bs{v} \, , \, p )_{\Om}
%%-\avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{v} }  }_{\G_I}
%%-( 1 \, , \,  p \, \nabla \cdot \bs{v} )_{\Om}
%%+ \avg{ \avgb{ p }_\lambda \, , \,    \jump{\bs{v} } }_{\G_I}
%%\nonumber \\
%%& \phantom{=} \;
%%{\color{red}
%%- \avg{p_{I}\, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\G_I}
%%- \avg{ \avgb{ \phi \, p }_\lambda \, , \,   t_{I} }_{\G_I}
%%}
%%\nonumber \\
%%&= \,
%%- \avg{p_{I}\, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\G_I}
%%- \avg{ \avgb{ \phi \, p }_\lambda \, , \,   t_{I} }_{\G_I}
%%\end{align}
%%which can be recast as
%%\begin{align}
%%\label{eq:SH_Cons3}
%%\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%%&=\;
%%	- \avg{ \jump{ p } \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\G_I}
%%- \avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{ \bs{v} } }_{\G_I}
%%+ \avg{ \jump{ p } - p_{I}\, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\G_I}
%%\nonumber \\
%%& \phantom{=} \;
%%+ \avg{ \jump{ \bs{v} } - t_{I} \, , \, \avgb{ \phi \, p }_\lambda  }_{\G_I}
%%\end{align}
%%or
%%\begin{align}
%%\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%%+ (1 \, , \, \nabla \cdot( \bs{v} \, p) )_{\Om}
%%&= \;
%% \avg{ \jump{ p } - p_{I}\, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\G_I}
%%+ \avg{ \jump{ \bs{v} } - t_{I} \, , \, \avgb{ \phi \, p }_\lambda  }_{\G_I}
%%\end{align}
%%\end{subequations}
%%%
%%
%%The case of the Shifted Interface Method is different, and in general it will not be possible to observe cancellation of fluxes over $\tGI$similar to the ones over $\G_I$ in~\eqref{eq:SH_Cons2}--\eqref{eq:SH_Cons3}.
%%This is because the SIM attempts to find approximations to the interface conditions on the true interface $\G_I$ using Taylor expansions of the field centered at points on $\tGI$.
%%Setting $\phi=0$ and $\bs{\psi}=\bs{e}_i$ in~\eqref{eq:SH_Weak7a}, we obtain
%%\begin{subequations}
%%\label{eq:SH_Cons4}
%%\begin{align}
%%\label{eq:SH_Cons4a}
%%\partial_t (1 \, , \, \rho \bs{v} \cdot \bs{e}_i)_{\Om}
%%&=\;
%%\avg{ \jump{(\nabla p ) \bs{d}} \, , \,   \avgb{ \bs{e}_i }_{1-\lambda}  }_{\tGI}
%%\; ,
%%\end{align}
%%%
%%which states that a small perturbation - of order $O(h)$ - to the momentum flux needs to be imposed on $\tGI$ to enforce the matching conditions~\eqref{eq:SBM_SH_IP} on the surrogate interface.
%%Analogously, setting $\phi=1$ in the energy equation and $\bs{\psi}=\bs{v}$ in the momentum equation, we obtain
%%%
%%\begin{align}
%%\label{eq:SH_Cons4b}
%%\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%%&=\;
%%\avg{ \jump{(\nabla p ) \bs{d}} {\color{red}-p_{I} \ti{\bs{n}}}  \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%%%
%%+ \avg{ \avgb{ p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, ( (\nabla \bs{v}) \bs{d}) - (\bs{\tau}_i \otimes \bs{\tau}_i) \, \bs{v}} -{\color{red}t_{I}} }_{\tGI}
%%\; ,
%%\nonumber \\
%%& = \;
%%\avg{ \jump{p + (\nabla p ) \bs{d}} -p_{I} \ti{\bs{n}} \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%%%
%%+\avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, (\bs{v} + (\nabla \bs{v}) \bs{d}) } -t_{I} }_{\tGI}
%%\nonumber \\
%%& \phantom{=} \;
%%- \avg{ \jump{ p } \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%%- \avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{ \bs{v} } }_{\tGI}
%%\end{align}
%%%
%%which can be recast as
%%%
%%\begin{align}
%%\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%%+ (1 \, , \, \nabla \cdot( \bs{v} \, p) )_{\Om}
%%& = \;
%%\avg{ \jump{p + (\nabla p ) \bs{d}} -p_{I} \ti{\bs{n}} \, , \,   \avgb{ \bs{v} }_{1-\lambda}  }_{\tGI}
%%\nonumber \\
%%& \phantom{=} \;
%%+\avg{ \avgb{ \phi \, p }_\lambda \, , \,    \jump{ ( \bs{n} \otimes \bs{n} )  \, (\bs{v} + (\nabla \bs{v}) \bs{d}) } -t_{I} }_{\tGI}
%%\nonumber \\
%%& = \;
%%O(h^2)
%%\end{align}
%%\end{subequations}
%%which indicates that a small, order $O(h^2)$, perturbation to the energy balance needs to be imposed to enforce the matching conditions~\eqref{eq:SBM_SH_IP}--\eqref{eq:SBM_SH_IN}.
%%This is of course expected, since the Taylor expansion is truncated to respect second-order accuracy.
%
%
%%--------------
%
%
%\subsection{A derivation of the shifted variational formulation through numerical fluxes}
%To summarize, the governing equations are
%\begin{subequations}
%	\label{eq:summay_strong_equations}
%	\begin{align}
%	\rho \dot{\bs{v}} + \nabla p &=  0\; , \label{momentumEq} \\
%	\rho \dot{{e}}  + \rho \, \dot{\bs{v}} \cdot \bs{v} &= 0 \; . \label{totalEnergyEq}
%	\end{align}
%\end{subequations}
%Substituting~\eqref{momentumEq} in~\eqref{totalEnergyEq}, equations~\eqref{eq:summay_strong_equations} can be equivalently written as
%\begin{subequations}
%	\label{eq:summay_strong_equations_p2}
%	\begin{align}
%	\rho \dot{\bs{v}} + \nabla p &=  0\; , \label{momentumEq_p2} \\
%	\rho \dot{{e}}  - \nabla p \cdot \bs{v} &= 0 \; . \label{totalEnergyEq_p2}
%	\end{align}
%\end{subequations}
%
%In deriving the shifted DG formulation, we will follow the typical steps of the local discontinuous Galerkin (LDG) formulation (see, e.g.,~\cite{arnold2002unified}, for more details). Multiplying the strong form of the equations~\eqref{momentumEq_p2}--\eqref{totalEnergyEq_p2}
%by the test function pair $[\phi \, , \, \bs{\psi}]$ and integrating over the generic element $T$ of the finite element mesh yield
%%
%\begin{subequations}
%	\begin{align}
%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{T}
%+ 	(\bs{\psi} \, , \, \nabla p )_{T}
%	=
%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{T}
%- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{T}
%	&
%	+  \langle p\, , \, \bs{\psi}\cdot \bs{n}  \rangle _{\partial T}
%	= 0
%	\, , \\
%(\phi \, , \, \rho \dot{e} )_{T}
%-
%(\nabla p \, , \,  \bs{v}\, \phi  )_{T}
%	& =
%(\phi \, , \, \rho \dot{e} )_{T}
%+ ( \nabla \cdot (\phi \, \bs{v}) \, , \,   p )_{T}
%-\langle\bs{v}\cdot\bs{n} \, , \, \phi \, p \rangle_{\partial T}
%	= \;
%0
%	\,.
%	\end{align}
%\end{subequations}
%%
%Replacing the boundary traces by suitable \textit{numerical fluxes}, $\hat{p}$ and $\hat{\bs{v}}$, yields
%%
%\begin{subequations}
%	\begin{align}
%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{T}
%- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{T}
%	+  \langle \hat{p}\, , \, \bs{\psi}\cdot\bs{n}  \rangle_{\partial T}
%	& = \;
%0
%	\, , \\
%(\phi \, , \, \rho \dot{e} )_{T}
%+ ( \nabla \cdot (\phi \, \bs{v}) \, , \,   p )_{T}
%-\langle \hat{\bs{v}}\cdot\bs{n} \, , \, \phi \, \hat{p} \rangle_{\partial T}
%	& = \;
%0\,.
%	\end{align}
%\end{subequations}
%%
%The numerical fluxes $\hat{p}$ and $\hat{\bs{v}}$ accomplish the linking of the numerical solution between neighboring elements, and will be defined momentarily. Summing over all the elements and integrating back by parts the second equation we have
%%
%\begin{subequations}
%	\label{eq:baseDG}
%	\begin{align}
%(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\sum_{T \in \ti{\mathcal{T}}^h} \langle \hat{p}\, , \, \bs{\psi}\cdot\bs{n}  \rangle _{\partial T}
%	& = \;
%0
%	\, , \\
%(\phi \, , \, \rho \dot{e} )_{\Om}
%- ( \nabla p \, , \,   \bs{v}\, \phi )_{\Om}
%-\sum_{T \in \ti{\mathcal{T}}^h} \langle \hat{\bs{v}} \cdot \bs{n} \, , \, \phi \, \hat{p}  \rangle _{\partial T}
%+ \sum_{T \in \ti{\mathcal{T}}^h} \langle \bs{v} \cdot \bs{n} \, , \, \phi \, p  \rangle _{\partial T}
%	& = \;
%0\,.
%	\end{align}
%\end{subequations}
%%
%%
%%
%%
%Next, we introduce the average operator $\avgb{ \cdot}_\gamma $ and the jump operator $\jump{\cdot}$
%for discontinuous scalars and vector fields across element boundaries:
%\begin{subequations}
%	\label{eq:jump_avg}
%	\begin{align}
%	\avgb{ p}_{\gamma}
%	&=\;
%	\gamma \, p^{+}+(1-\gamma ) \, p^{-}
%	\, , \quad \quad &
%	\avgb{ \bs{v}}_{\gamma}
%	&=\;
%	\gamma \,\bs{v}^{+}+(1-\gamma ) \,\bs{v}^{-}
%	\, ,  \qquad \, \, \,  \forall \gamma \in [0,1]
%	\, , \\
%	\jump{p}
%	&=
%	p^{+}\bs{n}^{+}+p^{-}\bs{n}^{-}
%	\, , \quad \quad &
%	\jump{\bs{v}}
%	&=\; \bs{v}^{+}\cdot\bs{n}^{+}+\bs{v}^{-}\cdot\bs{n}^{-}
%	\end{align}
%\end{subequations}
%%
%where $\bs{n}^{+}$ and $\bs{n}^{-}$  indicate opposite normals to a face.
%A reordering argument yields
%%
%\begin{equation}
%\sum_{T \in \ti{\mathcal{T}}^h} \avg{w\, , \, \bs{v}\cdot\bs{n} } _{\partial T}
%=
%\avg{ \avgb{ w }_{\gamma} \, , \, \jump{\bs{v}} }_{\tGI}
%+
%\avg{ \jump{ w } \, , \, \avgb{ \bs{v}}_{1-\gamma} }_{\tGI }
%+
%\avg{ w \, \bs{n} \, , \, \bs{v} } _{\partial \Om}
%\, ,
%\label{eq: identity property}
%\end{equation}
%%
%Using the definitions~\eqref{eq:jump_avg} of jump and average operators and inserting identity~\eqref{eq: identity property} into~\eqref{eq:baseDG}, we obtain
%%
%\begin{subequations}
%	\label{eq:dg_bf_intermediate}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_1}
%&(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\avg{ \avgb{ \hat{p}}_{\gamma} \, , \, \jump {\bs{\psi}} }_{\tGI}
%	+\avg{ \jump{ \hat{p}} \, , \, \avgb{ \bs{\psi}}_{1-\gamma} } _{\tGI}
%	+\avg{ \hat{p}\, , \, \bs{\psi} \cdot \bs{n} }_{\partial \Om}
%	= \;
%0
%	\,,\\
%	\label{eq:dg_bf_intermediate_2}
%&(\phi \, , \, \rho \dot{e} )_{\Om}
%- ( \nabla p \, , \,   \bs{v}\, \phi )_{\Om}
%-\avg{ \jump {\hat{\bs{v}} } \, , \,  \avgb{ \phi \, \hat{p} }_{\gamma} }_{\tGI }
%-\avg{  \avgb{\hat{\bs{v}}}_{1-\gamma}\, , \, \jump{ \phi \, \hat{p} } }_{\tGI }
%-\avg{  \hat{\bs{v}} \cdot \bs{n} \, , \,  \phi \, \hat{p} }_{\partial \Om}
%\nonumber \\
%& \phantom{=}
%+\avg{ \jump {\bs{v} } \, , \,  \avgb{ \phi \,p }_{\gamma} }_{\tGI }
%+\avg{  \avgb{\bs{v}}_{1-\gamma}\, , \, \jump{ \phi \, p } }_{\tGI }
%+\avg{   \bs{v}  \cdot \bs{n} \, , \,  \phi \, p }_{\partial \Om}
%= \;
%0
%	\, .
%	\end{align}
%\end{subequations}
%%
%%
%The sum of these equations will constitute the basis of the variational formulation.
%%
%%
%%
%Applying the LDG-type flux definitions~\cite{arnold2002unified} as a reference, we define the following {\it shifted} numerical fluxes on $\tGI$,
%%
%%\begin{array}{lll}
%\begin{equation}
%\begin{aligned}
%\hat{p}^{+}
%&=
%\avgb{ p}_{\gamma}
%- (1-\gamma) \, \jump{ \nabla p\cdot \bs{d} } \cdot \ti{\bs{n}}^{+}
%\; ,   \\
%\hat{p}^{-}
%&=
%\hat{p}^{+}
%+  \jump{ \nabla p \cdot \bs{d} } \cdot \ti{\bs{n}}^{+}
%\; ,   \\
%\hat{\bs{v}}^{+}
%&=
%\avgb{ \bs{v}}_{1-\gamma}
%- \gamma \jump{\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n} -  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i}  } \ti{\bs{n}}^{+}
%\; , \\
%\hat{\bs{v}}^{-}
%&=
%\hat{\bs{v}}^{+}
%+ \jump{\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n}
%	-  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i}  } \ti{\bs{n}}^{+}
%\, .
%%\end{array}
%\end{aligned}
%\end{equation}
%where $\bs{\tau}_i$ as a unit vector tangent to the true boundary surface (and we imply repeated index notation). In addition, we define $\hat{p}  = p$ and $\hat{\bs{v}} = 0 \,\bs{n}$ on $\partial \Om$.
%%
%Once these substitutions are made, the {\it discrete} variational form reads
%\begin{subequations}
%	\label{eq:dg_bf_intermediate_3}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_4}
%	&(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\avg{ \avgb{ p}_{\gamma} \, , \, \jump {\bs{\psi}} }_{\tGI}
%	-\avg{ \jump{ \nabla p \cdot \bs{d} } \, , \, \avgb{ \bs{\psi}}_{1-\gamma} } _{\tGI}
%   +\avg{ p \, , \, \bs{\psi} \cdot \bs{n} }_{\partial \Om}
%	= \;
%0
%	\,,\\
%	\label{eq:dg_bf_intermediate_5}
%	&(\phi \, , \, \rho \dot{e} )_{\Om}
%	- ( \nabla p \, , \,   \bs{v}\, \phi )_{\Om}
%	+\avg{ \jump {\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n}
%	-  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i} } \, , \,  \avgb{ \phi \, \hat{p} }_{\gamma} }_{\tGI }
%	-\avg{  \avgb{\bs{v}}_{1-\gamma}\, , \, \jump{ \phi \, \hat{p} } }_{\tGI }
%	+\avg{ \jump {\bs{v} } \, , \,  \avgb{ \phi \,p }_{\gamma} }_{\tGI }
%	\nonumber \\
%	& \phantom{=}
%	+\avg{  \avgb{\bs{v}}_{1-\gamma}\, , \, \jump{ \phi \, p } }_{\tGI }
%	+\avg{  \bs{v} \cdot \bs{n} \, , \,  \phi \, p }_{\partial \Om}
%	= \;
%0
%	\, .
%	\end{align}
%\end{subequations}
%%and the discrete trial and test spaces~\eqref{eq:finite_dimensional_function_spaces_Darcy} are introduced,
%Noting that $ \jump{ \phi \, p } =  \avgb{ \phi }_{1-\gamma} \, \jump{ p } + \jump{ \phi } \, \avgb{ p }_{\gamma} $, $ \jump{ \phi  } =  - \avgb{ \phi }_{1-\gamma}  \jump{ \nabla p \cdot \bs{d} }  + \jump{ \phi } \, \avgb{ p }_{\gamma}$ and $\avgb{ \phi \, \hat{p}} = \avgb{p}_{\gamma} \, \avgb{\phi}_{\gamma} - (1-\gamma) \, \gamma \, \jump{ \nabla p \cdot \bs{d} }  \cdot \jump{\phi}$, ~\eqref{eq:dg_bf_intermediate_3} can be rewritten as,
%\begin{subequations}
%	\label{eq:dg_bf_intermediate_6}
%	\begin{align}
%	\label{eq:dg_bf_intermediate_7}
%	&(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	- 	(\nabla \cdot \bs{\psi} \, , \,  p )_{\Om}
%	+\avg{ \avgb{ p}_{\gamma} \, , \, \jump {\bs{\psi}} }_{\tGI}
%	-\avg{ \jump{ \nabla p \cdot \bs{d} } \, , \, \avgb{ \bs{\psi}}_{1-\gamma} } _{\tGI}
%	+\avg{ p \, , \, \bs{\psi} \cdot \bs{n} }_{\partial \Om}
%	= \;
%	0
%	\,,\\
%	\label{eq:dg_bf_intermediate_8}
%	&(\phi \, , \, \rho \dot{e} )_{\Om}
%		- ( \nabla p \, , \,   \bs{v}\, \phi )_{\Om}
%	+\avg{ \jump {\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n}
%	-  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i} } \, , \,   \avgb{p}_{\gamma} \, \avgb{\phi}_{\gamma} -  (1-\gamma) \, \gamma \, \left( \jump{ \nabla p \cdot \bs{d} } \right) \cdot \jump{\phi} }_{\tGI }
%	\nonumber \\
%	& \phantom{=}
%	+\avg{  \avgb{\bs{v}}_{1-\gamma}\, , \, \avgb{ \phi }_{1-\gamma} \, \jump{ p + \nabla p \cdot \bs{d} }   }_{\tGI }
%	+\avg{ \jump {\bs{v} } \, , \,  \avgb{ \phi \,p }_{\gamma} }_{\tGI }
%	+\avg{  \bs{v} \cdot \bs{n} \, , \,  \phi \, p }_{\partial \Om}
%	= \;
%	0
%	\, .
%	\end{align}
%\end{subequations}
%
%\subsubsection{Conservation properties}
%%\subsubsection{Equations~\eqref{eq:dg_bf_intermediate_6}}
%
%To start the discussion, let us consider a body-fitted variational formulation that corresponds to the limit case of the SIM when $\bs{d} \rightarrow \bs{0}$, so that $\tGI \rightarrow \G_I$, $\ti{\bs{n}} \rightarrow \bs{n}$, $\ti{\bs{n}} \cdot \bs{n} = 1$ and $\ti{\bs{n}} \cdot \bs{\tau}_i = 0$.
%In this limit, \eqref{eq:dg_bf_intermediate_6} reduce to:
%%
%\begin{subequations}
%	\label{eq:SH_Cons1-V2}
%	\begin{align}
%	&	(\bs{\psi} \, , \, \rho \dot{\bs{v}})_{\Om}
%	-
%	(\nabla \cdot \bs{\psi} \, , \, p )_{\Om}
%	+\avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{\psi} }  }_{\G_I}
%	+\avg{ p \, , \, \bs{\psi} \cdot \bs{n} }_{\partial \Om}
%	=\;
%	0 \; ,
%	\\
%	&	(\phi \, , \, \rho \dot{e} )_{\Om}
%	- ( \nabla p \, , \,   \bs{v}\, \phi )_{\Om}
%	+\avg{  \avgb{\bs{v}}_{1-\lambda}\, , \, \avgb{ \phi }_{1-\lambda}  \jump{ p } }_{\G_I }
%	+\avg{ \jump {\bs{v} } \, , \,  \avgb{ \phi \,p }_{\lambda} }_{\G_I}
%	+\avg{  \bs{v} \cdot \bs{n} \, , \,  \phi \, p }_{\partial \Om}
%	= \;
%	0 .
%	\end{align}
%\end{subequations}
%%
%%
%The global statement of conservation of total energy is obtained setting $\phi=1$ in the energy equation, $\bs{\psi}=\bs{v}$ in the momentum equation (to obtain a kinetic energy balance). Integrating by parts the second equation and summing the results,
%%
%	\begin{align}
%	\label{eq:SH_Cons3a-V2}
%	\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%	&=\;
%	- \avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{v} } - 0 \, \bs{n}  }_{\G_I}
%	+\avg{ p \, , \, \bs{v} \cdot \bs{n} - 0}_{\partial \Om}
%	\end{align}
%%
%Analogously, setting $\phi=1$ and $\bs{\psi}=\bs{v}$ in \eqref{eq:dg_bf_intermediate_6}, integrating by parts the second equation and summing the results, we obtain
%%
%	\begin{align}
%	\label{eq:SH_Cons4b-V2}
%	\partial_t (1 \, , \, \rho ( \bs{v} \cdot \bs{v} /2 + e) )_{\Om}
%	&=
%	- \avg{ \avgb{ p }_\lambda \, , \,  \ljump{ \bs{v} }  }_{\tGI}
%	-\avg{ \jump {\left( (\nabla \bs{v} \, \bs{d})\cdot \bs{n} \right) \bs{n}
%		-  \left( \bs{v} \cdot \bs{\tau}_{i} \right) \bs{\tau}_{i} } \, , \,   \avgb{p}_{\gamma} }_{\tGI }
%	+\avg{ p \, , \, \bs{v} \cdot \bs{n} }_{\partial \Om}
%	\nonumber \\
%	& =
%	-\avg{ \jump {  ( \bs{n} \otimes \bs{n} )  \, (\bs{v} + (\nabla \bs{v}) \bs{d})  } - 0 \, \left( \bs{n}\cdot \ti{\bs{n}} \right)\, , \,   \avgb{p}_{\lambda} }_{\tGI }
%	+\avg{ p \, , \, \bs{v} \cdot \bs{n} - 0 }_{\partial \Om}
%	\end{align}
%	%
%which indicates that a small, order $O(h^2)$, perturbation to the energy balance needs to be imposed to enforce the matching conditions~\eqref{eq:SBM_SH_IP}--\eqref{eq:SBM_SH_IN}.
%This is of course expected, since the Taylor expansion is truncated to respect second-order accuracy.

